On the Robustness of Winners: Counting Briberies in Elections

We study the parameterized complexity of counting variants of Swap- and Shift-Bribery problems, focusing on the parameterizations by the number of swaps and the number of voters. We show experimentally that Swap-Bribery offers a new approach to the robustness analysis of elections.

==> id110.tex <==
\begin{axis}[anchor=north, no markers, enlargelimits=false, legend columns=2, 
legend style={draw=none,/tikz/column 2/.style={column sep=5pt,},}, every axis 
plot/.append style={ultra thick}, legend style = 
{font=\LARGE,fill=none},ticklabel style={font=\LARGE},title 
style={font=\LARGE},cycle list name=color list, ytick={0,0.2,0.4,0.6,0.8,1}, 
yticklabels={,0.2,0.4,0.6,0.8,1}, title= 3D Cube, label style={font=\huge}, 
ylabel shift = 3pt, ylabel=$P_c(r)$
]
\addplot+[lightgray,forget plot, thick] coordinates{(0,0.5) (0.5,0.5)};
\addplot[red]coordinates{(0.0, 1.0) (0.0125, 0.6393) (0.025, 0.4908) (0.037500000000000006, 0.4143) (0.05, 0.3475) (0.0625, 0.3014) (0.07500000000000001, 0.2564) (0.08750000000000001, 0.221) (0.1, 0.1916) (0.1125, 0.1672) (0.125, 0.1585) (0.1375, 0.143) (0.15000000000000002, 0.1396) (0.1625, 0.128) (0.17500000000000002, 0.1203) (0.1875, 0.1182) (0.2, 0.1124) (0.21250000000000002, 0.113) (0.225, 0.1127) (0.23750000000000002, 0.1146) (0.25, 0.1201) (0.2625, 0.1152) (0.275, 0.1178) (0.28750000000000003, 0.1274) (0.30000000000000004, 0.1248) (0.3125, 0.129) (0.325, 0.1323) (0.3375, 0.1365) (0.35000000000000003, 0.1341) (0.36250000000000004, 0.1506) (0.375, 0.1473) (0.3875, 0.1504) (0.4, 0.1588) (0.41250000000000003, 0.1527) (0.42500000000000004, 0.1575) (0.4375, 0.1507) (0.45, 0.1511) (0.4625, 0.1357) (0.47500000000000003, 0.1414) (0.48750000000000004, 0.1367) (0.5, 0.1262)};
\addlegendentry{17/530/1}
\addplot[blue]coordinates{(0.0, 0.0) (0.0125, 0.4501) (0.025, 0.4934) (0.037500000000000006, 0.5087) (0.05, 0.5017) (0.0625, 0.4765) (0.07500000000000001, 0.4377) (0.08750000000000001, 0.4036) (0.1, 0.3689) (0.1125, 0.3306) (0.125, 0.2959) (0.1375, 0.272) (0.15000000000000002, 0.2546) (0.1625, 0.2317) (0.17500000000000002, 0.2151) (0.1875, 0.2101) (0.2, 0.1901) (0.21250000000000002, 0.1799) (0.225, 0.1754) (0.23750000000000002, 0.1632) (0.25, 0.1591) (0.2625, 0.1568) (0.275, 0.1504) (0.28750000000000003, 0.1486) (0.30000000000000004, 0.1512) (0.3125, 0.1539) (0.325, 0.1427) (0.3375, 0.1426) (0.35000000000000003, 0.1511) (0.36250000000000004, 0.1433) (0.375, 0.1501) (0.3875, 0.1483) (0.4, 0.1469) (0.41250000000000003, 0.1476) (0.42500000000000004, 0.1443) (0.4375, 0.1444) (0.45, 0.1433) (0.4625, 0.137) (0.47500000000000003, 0.1337) (0.48750000000000004, 0.1325) (0.5, 0.1245)};
\addlegendentry{16/500/2}
\addplot[black]coordinates{(0.0, 0.0) (0.0125, 0.264) (0.025, 0.2371) (0.037500000000000006, 0.2131) (0.05, 0.1768) (0.0625, 0.1447) (0.07500000000000001, 0.1177) (0.08750000000000001, 0.0945) (0.1, 0.0743) (0.1125, 0.0654) (0.125, 0.0584) (0.1375, 0.0497) (0.15000000000000002, 0.0414) (0.1625, 0.0375) (0.17500000000000002, 0.0383) (0.1875, 0.0348) (0.2, 0.0343) (0.21250000000000002, 0.0372) (0.225, 0.0337) (0.23750000000000002, 0.0344) (0.25, 0.0375) (0.2625, 0.0429) (0.275, 0.0424) (0.28750000000000003, 0.0403) (0.30000000000000004, 0.0482) (0.3125, 0.0506) (0.325, 0.0572) (0.3375, 0.0587) (0.35000000000000003, 0.0662) (0.36250000000000004, 0.07) (0.375, 0.0741) (0.3875, 0.0806) (0.4, 0.0894) (0.41250000000000003, 0.0921) (0.42500000000000004, 0.1031) (0.4375, 0.109) (0.45, 0.1091) (0.4625, 0.1195) (0.47500000000000003, 0.1237) (0.48750000000000004, 0.1256) (0.5, 0.1259)};
\addlegendentry{16/445/2}
\addplot[black!30!green]coordinates{(0.0, 0.0) (0.0125, 0.0005) (0.025, 0.0091) (0.037500000000000006, 0.0461) (0.05, 0.109) (0.0625, 0.1865) (0.07500000000000001, 0.2729) (0.08750000000000001, 0.344) (0.1, 0.3968) (0.1125, 0.4579) (0.125, 0.5033) (0.1375, 0.5427) (0.15000000000000002, 0.564) (0.1625, 0.5913) (0.17500000000000002, 0.6048) (0.1875, 0.6163) (0.2, 0.6367) (0.21250000000000002, 0.6418) (0.225, 0.6342) (0.23750000000000002, 0.6407) (0.25, 0.635) (0.2625, 0.6285) (0.275, 0.6179) (0.28750000000000003, 0.6023) (0.30000000000000004, 0.5973) (0.3125, 0.5748) (0.325, 0.5613) (0.3375, 0.5318) (0.35000000000000003, 0.5107) (0.36250000000000004, 0.478) (0.375, 0.4509) (0.3875, 0.4208) (0.4, 0.3892) (0.41250000000000003, 0.3698) (0.42500000000000004, 0.3208) (0.4375, 0.2875) (0.45, 0.2572) (0.4625, 0.2201) (0.47500000000000003, 0.1852) (0.48750000000000004, 0.1601) (0.5, 0.123)};
\addlegendentry{8/690/7}
\end{axis}

==> id149.tex <==
\begin{axis}[anchor=north, no markers, enlargelimits=false, legend columns=2, 
legend style={draw=none,/tikz/column 2/.style={column sep=5pt,},}, every axis 
plot/.append style={ultra thick}, legend style = 
{font=\LARGE,fill=none},ticklabel style={font=\LARGE},title 
style={font=\LARGE},cycle list name=color list, ytick={0,0.2,0.4,0.6,0.8,1}, 
yticklabels={,0.2,0.4,0.6,0.8,1}, title= 5D Cube, xlabel=$r$,xlabel shift = 
4pt, label 
style={font=\huge}
]
\addplot+[lightgray,forget plot, thick] coordinates{(0,0.5) (0.5,0.5)};
\addplot[red]coordinates{(0.0, 1.0) (0.0125, 0.8386) (0.025, 0.6242) 
(0.037500000000000006, 0.4666) (0.05, 0.3793) (0.0625, 0.3043) 
(0.07500000000000001, 0.2509) (0.08750000000000001, 0.2122) (0.1, 0.1824) 
(0.1125, 0.1625) (0.125, 0.1506) (0.1375, 0.1345) (0.15000000000000002, 0.1161) 
(0.1625, 0.1185) (0.17500000000000002, 0.107) (0.1875, 0.0991) (0.2, 0.1) 
(0.21250000000000002, 0.0897) (0.225, 0.0906) (0.23750000000000002, 0.0944) 
(0.25, 0.0915) (0.2625, 0.0921) (0.275, 0.0893) (0.28750000000000003, 0.0883) 
(0.30000000000000004, 0.0929) (0.3125, 0.0941) (0.325, 0.0906) (0.3375, 0.0977) 
(0.35000000000000003, 0.0992) (0.36250000000000004, 0.1018) (0.375, 0.1026) 
(0.3875, 0.1013) (0.4, 0.1102) (0.41250000000000003, 0.1141) 
(0.42500000000000004, 0.1079) (0.4375, 0.1164) (0.45, 0.1162) (0.4625, 0.1161) 
(0.47500000000000003, 0.1201) (0.48750000000000004, 0.1225) (0.5, 0.1247)};
\addlegendentry{20/443/1}
\addplot[blue]coordinates{(0.0, 0.0) (0.0125, 0.2831) (0.025, 0.4818) (0.037500000000000006, 0.5943) (0.05, 0.6505) (0.0625, 0.699) (0.07500000000000001, 0.7326) (0.08750000000000001, 0.746) (0.1, 0.7623) (0.1125, 0.7687) (0.125, 0.7743) (0.1375, 0.7752) (0.15000000000000002, 0.7754) (0.1625, 0.7666) (0.17500000000000002, 0.7657) (0.1875, 0.7559) (0.2, 0.7446) (0.21250000000000002, 0.74) (0.225, 0.7179) (0.23750000000000002, 0.7047) (0.25, 0.6952) (0.2625, 0.6746) (0.275, 0.6631) (0.28750000000000003, 0.6476) (0.30000000000000004, 0.6114) (0.3125, 0.5929) (0.325, 0.5649) (0.3375, 0.5307) (0.35000000000000003, 0.5022) (0.36250000000000004, 0.479) (0.375, 0.4465) (0.3875, 0.407) (0.4, 0.3738) (0.41250000000000003, 0.3457) (0.42500000000000004, 0.3099) (0.4375, 0.2759) (0.45, 0.2525) (0.4625, 0.2142) (0.47500000000000003, 0.1809) (0.48750000000000004, 0.1563) (0.5, 0.1248)};
\addlegendentry{17/661/2}
\addplot[black]coordinates{(0.0, 0.0) (0.0125, 0.0211) (0.025, 0.0614) (0.037500000000000006, 0.0943) (0.05, 0.1086) (0.0625, 0.1212) (0.07500000000000001, 0.1344) (0.08750000000000001, 0.1362) (0.1, 0.1406) (0.1125, 0.1485) (0.125, 0.1474) (0.1375, 0.1535) (0.15000000000000002, 0.1637) (0.1625, 0.1607) (0.17500000000000002, 0.1677) (0.1875, 0.1665) (0.2, 0.1746) (0.21250000000000002, 0.1755) (0.225, 0.1811) (0.23750000000000002, 0.1809) (0.25, 0.1777) (0.2625, 0.1877) (0.275, 0.1848) (0.28750000000000003, 0.1908) (0.30000000000000004, 0.1903) (0.3125, 0.1928) (0.325, 0.2003) (0.3375, 0.1937) (0.35000000000000003, 0.1929) (0.36250000000000004, 0.1979) (0.375, 0.1875) (0.3875, 0.1915) (0.4, 0.1831) (0.41250000000000003, 0.175) (0.42500000000000004, 0.1768) (0.4375, 0.1781) (0.45, 0.1578) (0.4625, 0.1521) (0.47500000000000003, 0.1488) (0.48750000000000004, 0.1356) (0.5, 0.1299)};
\addlegendentry{16/536/3}
\addplot[black!30!green]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0001) (0.037500000000000006, 0.0003) (0.05, 0.0019) (0.0625, 0.003) (0.07500000000000001, 0.0058) (0.08750000000000001, 0.0107) (0.1, 0.0137) (0.1125, 0.0219) (0.125, 0.0224) (0.1375, 0.0293) (0.15000000000000002, 0.0337) (0.1625, 0.0384) (0.17500000000000002, 0.0503) (0.1875, 0.0534) (0.2, 0.0572) (0.21250000000000002, 0.0643) (0.225, 0.0773) (0.23750000000000002, 0.0825) (0.25, 0.0948) (0.2625, 0.1003) (0.275, 0.1048) (0.28750000000000003, 0.114) (0.30000000000000004, 0.1249) (0.3125, 0.1363) (0.325, 0.1371) (0.3375, 0.1421) (0.35000000000000003, 0.1526) (0.36250000000000004, 0.1548) (0.375, 0.167) (0.3875, 0.1603) (0.4, 0.1649) (0.41250000000000003, 0.1656) (0.42500000000000004, 0.165) (0.4375, 0.1611) (0.45, 0.1547) (0.4625, 0.1509) (0.47500000000000003, 0.1425) (0.48750000000000004, 0.1375) (0.5, 0.1269)};
\addlegendentry{10/536/4}
\end{axis}

==> id20.tex <==
\begin{axis}[anchor=north, no markers, enlargelimits=false, legend columns=2, legend style={draw=none,/tikz/column 2/.style={column sep=5pt,},}, every axis plot/.append style={ultra thick}, legend style = {font=\LARGE,fill=none},ticklabel style={font=\LARGE},title style={font=\LARGE},cycle list name=color list, ytick={0,0.2,0.4,0.6,0.8,1}, yticklabels={,0.2,0.4,0.6,0.8,1}, title= Impartial Culture
]
\addplot+[lightgray,forget plot, thick] coordinates{(0,0.5) (0.4,0.5)};
\addplot[red]coordinates{(0.0, 1.0) (0.0125, 0.8791) (0.025, 0.7364) (0.037500000000000006, 0.6476) (0.05, 0.5834) (0.0625, 0.5234) (0.07500000000000001, 0.4863) (0.08750000000000001, 0.4464) (0.1, 0.4128) (0.1125, 0.3758) (0.125, 0.3713) (0.1375, 0.3433) (0.15000000000000002, 0.3198) (0.1625, 0.3055) (0.17500000000000002, 0.295) (0.1875, 0.2773) (0.2, 0.2604) (0.21250000000000002, 0.2505) (0.225, 0.2286) (0.23750000000000002, 0.2331) (0.25, 0.2179) (0.2625, 0.203) (0.275, 0.1964) (0.28750000000000003, 0.1867) (0.30000000000000004, 0.1834) (0.3125, 0.1665) (0.325, 0.1707) (0.3375, 0.1545) (0.35000000000000003, 0.1555) (0.36250000000000004, 0.1476) (0.375, 0.1513) (0.3875, 0.1393) (0.4, 0.1348) (0.41250000000000003, 0.1293) (0.42500000000000004, 0.1311) (0.4375, 0.1218) (0.45, 0.1144) (0.4625, 0.1129) (0.47500000000000003, 0.1092) (0.48750000000000004, 0.1073) (0.5, 0.1022)};
\addlegendentry{470/1}
\addplot[blue]coordinates{(0.0, 0.0) (0.0125, 0.1299) (0.025, 0.1939) (0.037500000000000006, 0.208) (0.05, 0.2178) (0.0625, 0.2273) (0.07500000000000001, 0.2223) (0.08750000000000001, 0.2271) (0.1, 0.2202) (0.1125, 0.217) (0.125, 0.2073) (0.1375, 0.2118) (0.15000000000000002, 0.1977) (0.1625, 0.1918) (0.17500000000000002, 0.1822) (0.1875, 0.1854) (0.2, 0.1815) (0.21250000000000002, 0.1784) (0.225, 0.1671) (0.23750000000000002, 0.1619) (0.25, 0.1682) (0.2625, 0.1681) (0.275, 0.1518) (0.28750000000000003, 0.1517) (0.30000000000000004, 0.1488) (0.3125, 0.149) (0.325, 0.1409) (0.3375, 0.1448) (0.35000000000000003, 0.1363) (0.36250000000000004, 0.1394) (0.375, 0.1302) (0.3875, 0.1295) (0.4, 0.1253) (0.41250000000000003, 0.1248) (0.42500000000000004, 0.1192) (0.4375, 0.1161) (0.45, 0.1126) (0.4625, 0.112) (0.47500000000000003, 0.1077) (0.48750000000000004, 0.1063) (0.5, 0.1049)};
\addlegendentry{464/2}
\addplot[black]coordinates{(0.0, 0.0) (0.0125, 0.0354) (0.025, 0.092) (0.037500000000000006, 0.1217) (0.05, 0.1424) (0.0625, 0.1494) (0.07500000000000001, 0.1577) (0.08750000000000001, 0.1695) (0.1, 0.1728) (0.1125, 0.1786) (0.125, 0.1761) (0.1375, 0.1658) (0.15000000000000002, 0.1698) (0.1625, 0.1666) (0.17500000000000002, 0.1699) (0.1875, 0.1636) (0.2, 0.1599) (0.21250000000000002, 0.1548) (0.225, 0.157) (0.23750000000000002, 0.1511) (0.25, 0.1474) (0.2625, 0.1408) (0.275, 0.1462) (0.28750000000000003, 0.1401) (0.30000000000000004, 0.1367) (0.3125, 0.1386) (0.325, 0.1348) (0.3375, 0.1306) (0.35000000000000003, 0.1335) (0.36250000000000004, 0.1278) (0.375, 0.1194) (0.3875, 0.1185) (0.4, 0.1179) (0.41250000000000003, 0.1209) (0.42500000000000004, 0.1134) (0.4375, 0.1161) (0.45, 0.1151) (0.4625, 0.1072) (0.47500000000000003, 0.1072) (0.48750000000000004, 0.1045) (0.5, 0.1026)};
\addlegendentry{461/3}
\addplot[black!30!green]coordinates{(0.0, 0.0) (0.0125, 0.0049) (0.025, 0.0259) (0.037500000000000006, 0.0462) (0.05, 0.0556) (0.0625, 0.0657) (0.07500000000000001, 0.0707) (0.08750000000000001, 0.0761) (0.1, 0.085) (0.1125, 0.0909) (0.125, 0.0899) (0.1375, 0.1021) (0.15000000000000002, 0.0963) (0.1625, 0.1092) (0.17500000000000002, 0.1144) (0.1875, 0.1045) (0.2, 0.1083) (0.21250000000000002, 0.1152) (0.225, 0.1114) (0.23750000000000002, 0.1189) (0.25, 0.1155) (0.2625, 0.117) (0.275, 0.1177) (0.28750000000000003, 0.1184) (0.30000000000000004, 0.1132) (0.3125, 0.123) (0.325, 0.1137) (0.3375, 0.118) (0.35000000000000003, 0.1176) (0.36250000000000004, 0.115) (0.375, 0.1169) (0.3875, 0.1125) (0.4, 0.1184) (0.41250000000000003, 0.1071) (0.42500000000000004, 0.1093) (0.4375, 0.1116) (0.45, 0.111) (0.4625, 0.104) (0.47500000000000003, 0.1036) (0.48750000000000004, 0.1013) (0.5, 0.1027)};
\addlegendentry{458/4}
\end{axis}

==> id255.tex <==
\begin{axis}[anchor=north, no markers, enlargelimits=false, legend columns=2, legend style={draw=none,/tikz/column 2/.style={column sep=5pt,},}, every axis plot/.append style={ultra thick}, legend style = {font=\LARGE,fill=none},ticklabel style={font=\LARGE},title style={font=\LARGE},cycle list name=color list, ytick={0,0.2,0.4,0.6,0.8,1}, yticklabels={,0.2,0.4,0.6,0.8,1}, title= 3D Sphere
]
\addplot+[lightgray,forget plot, thick] coordinates{(0,0.5) (0.5,0.5)};
\addplot[red]coordinates{(0.0, 1.0) (0.0125, 0.7777) (0.025, 0.6538) (0.037500000000000006, 0.5954) (0.05, 0.5419) (0.0625, 0.5019) (0.07500000000000001, 0.4561) (0.08750000000000001, 0.431) (0.1, 0.4071) (0.1125, 0.3844) (0.125, 0.372) (0.1375, 0.3531) (0.15000000000000002, 0.3438) (0.1625, 0.3182) (0.17500000000000002, 0.319) (0.1875, 0.3022) (0.2, 0.2845) (0.21250000000000002, 0.2818) (0.225, 0.2739) (0.23750000000000002, 0.2716) (0.25, 0.2588) (0.2625, 0.2508) (0.275, 0.2417) (0.28750000000000003, 0.2361) (0.30000000000000004, 0.2269) (0.3125, 0.2189) (0.325, 0.2159) (0.3375, 0.2043) (0.35000000000000003, 0.2033) (0.36250000000000004, 0.1925) (0.375, 0.1786) (0.3875, 0.1757) (0.4, 0.1713) (0.41250000000000003, 0.1628) (0.42500000000000004, 0.1612) (0.4375, 0.1499) (0.45, 0.1467) (0.4625, 0.1452) (0.47500000000000003, 0.1386) (0.48750000000000004, 0.1278) (0.5, 0.1297)};
\addlegendentry{16/494/1}
\addplot[blue]coordinates{(0.0, 0.0) (0.0125, 0.4016) (0.025, 0.4179) (0.037500000000000006, 0.4082) (0.05, 0.3891) (0.0625, 0.3617) (0.07500000000000001, 0.3311) (0.08750000000000001, 0.3086) (0.1, 0.2885) (0.1125, 0.2703) (0.125, 0.2483) (0.1375, 0.2507) (0.15000000000000002, 0.2217) (0.1625, 0.2146) (0.17500000000000002, 0.2042) (0.1875, 0.2055) (0.2, 0.1942) (0.21250000000000002, 0.1825) (0.225, 0.1722) (0.23750000000000002, 0.1637) (0.25, 0.1651) (0.2625, 0.1598) (0.275, 0.1562) (0.28750000000000003, 0.1513) (0.30000000000000004, 0.1475) (0.3125, 0.1461) (0.325, 0.1375) (0.3375, 0.1409) (0.35000000000000003, 0.1386) (0.36250000000000004, 0.136) (0.375, 0.1303) (0.3875, 0.1239) (0.4, 0.134) (0.41250000000000003, 0.1324) (0.42500000000000004, 0.1229) (0.4375, 0.1243) (0.45, 0.1227) (0.4625, 0.1266) (0.47500000000000003, 0.1247) (0.48750000000000004, 0.1252) (0.5, 0.1247)};
\addlegendentry{15/449/2}
\addplot[black]coordinates{(0.0, 0.0) (0.0125, 0.002) (0.025, 0.0152) (0.037500000000000006, 0.0402) (0.05, 0.0698) (0.0625, 0.0979) (0.07500000000000001, 0.1185) (0.08750000000000001, 0.1386) (0.1, 0.1502) (0.1125, 0.1681) (0.125, 0.18) (0.1375, 0.1801) (0.15000000000000002, 0.1924) (0.1625, 0.2009) (0.17500000000000002, 0.1973) (0.1875, 0.1929) (0.2, 0.2039) (0.21250000000000002, 0.2028) (0.225, 0.1994) (0.23750000000000002, 0.2132) (0.25, 0.2006) (0.2625, 0.1968) (0.275, 0.1887) (0.28750000000000003, 0.1896) (0.30000000000000004, 0.1847) (0.3125, 0.1769) (0.325, 0.1793) (0.3375, 0.1752) (0.35000000000000003, 0.1683) (0.36250000000000004, 0.1575) (0.375, 0.1614) (0.3875, 0.1554) (0.4, 0.1505) (0.41250000000000003, 0.1482) (0.42500000000000004, 0.1529) (0.4375, 0.1387) (0.45, 0.137) (0.4625, 0.1391) (0.47500000000000003, 0.1292) (0.48750000000000004, 0.1256) (0.5, 0.1231)};
\addlegendentry{10/477/5}
\addplot[black!30!green]coordinates{(0.0, 0.0) (0.0125, 0.003) (0.025, 0.0169) (0.037500000000000006, 0.0397) (0.05, 0.0711) (0.0625, 0.0892) (0.07500000000000001, 0.1054) (0.08750000000000001, 0.1202) (0.1, 0.1343) (0.1125, 0.1451) (0.125, 0.1535) (0.1375, 0.1572) (0.15000000000000002, 0.1667) (0.1625, 0.172) (0.17500000000000002, 0.1711) (0.1875, 0.1763) (0.2, 0.1756) (0.21250000000000002, 0.1761) (0.225, 0.1732) (0.23750000000000002, 0.1802) (0.25, 0.1705) (0.2625, 0.168) (0.275, 0.1743) (0.28750000000000003, 0.1669) (0.30000000000000004, 0.1691) (0.3125, 0.1683) (0.325, 0.1598) (0.3375, 0.159) (0.35000000000000003, 0.1562) (0.36250000000000004, 0.1663) (0.375, 0.1555) (0.3875, 0.1548) (0.4, 0.1539) (0.41250000000000003, 0.1432) (0.42500000000000004, 0.1388) (0.4375, 0.1466) (0.45, 0.1333) (0.4625, 0.129) (0.47500000000000003, 0.1293) (0.48750000000000004, 0.1289) (0.5, 0.1241)};
\addlegendentry{10/476/5}
\end{axis}

==> id307.tex <==
\begin{axis}[anchor=north, no markers, enlargelimits=false, legend columns=2, 
legend style={draw=none,/tikz/column 2/.style={column sep=5pt,},}, every axis 
plot/.append style={ultra thick}, legend style = 
{font=\LARGE,fill=none},ticklabel style={font=\LARGE},title 
style={font=\LARGE},cycle list name=color list, ytick={0,0.2,0.4,0.6,0.8,1}, 
yticklabels={,0.2,0.4,0.6,0.8,1}, title= SPOC, xlabel=$r$,xlabel shift = 4pt, 
label style={font=\huge}
]
\addplot+[lightgray,forget plot, thick] coordinates{(0,0.5) (0.4,0.5)};
\addplot[red]coordinates{(0.0, 1.0) (0.0125, 0.4665) (0.025, 0.3655) (0.037500000000000006, 0.3258) (0.05, 0.2818) (0.0625, 0.2635) (0.07500000000000001, 0.2343) (0.08750000000000001, 0.2337) (0.1, 0.2204) (0.1125, 0.205) (0.125, 0.196) (0.1375, 0.1946) (0.15000000000000002, 0.1845) (0.1625, 0.1828) (0.17500000000000002, 0.173) (0.1875, 0.1675) (0.2, 0.1658) (0.21250000000000002, 0.1553) (0.225, 0.1618) (0.23750000000000002, 0.1596) (0.25, 0.1568) (0.2625, 0.1556) (0.275, 0.1499) (0.28750000000000003, 0.1471) (0.30000000000000004, 0.145) (0.3125, 0.1381) (0.325, 0.1373) (0.3375, 0.1367) (0.35000000000000003, 0.1279) (0.36250000000000004, 0.1354) (0.375, 0.1222) (0.3875, 0.1269) (0.4, 0.1238) (0.41250000000000003, 0.1187) (0.42500000000000004, 0.1153) (0.4375, 0.1124) (0.45, 0.1145) (0.4625, 0.1104) (0.47500000000000003, 0.1112) (0.48750000000000004, 0.1034) (0.5, 0.1025)};
\addlegendentry{462/1}
\addplot[blue]coordinates{(0.0, 0.0) (0.0125, 0.4176) (0.025, 0.386) (0.037500000000000006, 0.3602) (0.05, 0.3345) (0.0625, 0.3223) (0.07500000000000001, 0.3065) (0.08750000000000001, 0.2852) (0.1, 0.2615) (0.1125, 0.2605) (0.125, 0.2489) (0.1375, 0.2419) (0.15000000000000002, 0.2178) (0.1625, 0.223) (0.17500000000000002, 0.2113) (0.1875, 0.1934) (0.2, 0.1858) (0.21250000000000002, 0.18) (0.225, 0.1739) (0.23750000000000002, 0.1713) (0.25, 0.1642) (0.2625, 0.1555) (0.275, 0.1505) (0.28750000000000003, 0.1493) (0.30000000000000004, 0.1389) (0.3125, 0.144) (0.325, 0.1383) (0.3375, 0.1337) (0.35000000000000003, 0.1295) (0.36250000000000004, 0.1284) (0.375, 0.1262) (0.3875, 0.1255) (0.4, 0.1265) (0.41250000000000003, 0.1164) (0.42500000000000004, 0.1188) (0.4375, 0.1121) (0.45, 0.1126) (0.4625, 0.1079) (0.47500000000000003, 0.1031) (0.48750000000000004, 0.1017) (0.5, 0.1023)};
\addlegendentry{461/2}
\addplot[black]coordinates{(0.0, 0.0) (0.0125, 0.1761) (0.025, 0.1983) (0.037500000000000006, 0.1937) (0.05, 0.1941) (0.0625, 0.1902) (0.07500000000000001, 0.1875) (0.08750000000000001, 0.1888) (0.1, 0.1825) (0.1125, 0.1694) (0.125, 0.173) (0.1375, 0.1717) (0.15000000000000002, 0.1671) (0.1625, 0.1509) (0.17500000000000002, 0.1612) (0.1875, 0.1524) (0.2, 0.1581) (0.21250000000000002, 0.1494) (0.225, 0.1395) (0.23750000000000002, 0.146) (0.25, 0.1358) (0.2625, 0.1383) (0.275, 0.1353) (0.28750000000000003, 0.1302) (0.30000000000000004, 0.1343) (0.3125, 0.1304) (0.325, 0.1273) (0.3375, 0.1238) (0.35000000000000003, 0.1273) (0.36250000000000004, 0.1239) (0.375, 0.1211) (0.3875, 0.1174) (0.4, 0.1134) (0.41250000000000003, 0.1178) (0.42500000000000004, 0.116) (0.4375, 0.1145) (0.45, 0.1072) (0.4625, 0.1053) (0.47500000000000003, 0.1055) (0.48750000000000004, 0.1048) (0.5, 0.1081)};
\addlegendentry{459/3}
\addplot[black!30!green]coordinates{(0.0, 0.0) (0.0125, 0.0585) (0.025, 0.1103) (0.037500000000000006, 0.1384) (0.05, 0.1557) (0.0625, 0.1592) (0.07500000000000001, 0.1613) (0.08750000000000001, 0.1531) (0.1, 0.1663) (0.1125, 0.1598) (0.125, 0.1653) (0.1375, 0.1522) (0.15000000000000002, 0.1513) (0.1625, 0.1526) (0.17500000000000002, 0.1402) (0.1875, 0.1439) (0.2, 0.1349) (0.21250000000000002, 0.1433) (0.225, 0.1346) (0.23750000000000002, 0.1343) (0.25, 0.1313) (0.2625, 0.1331) (0.275, 0.131) (0.28750000000000003, 0.127) (0.30000000000000004, 0.1195) (0.3125, 0.1258) (0.325, 0.1247) (0.3375, 0.1212) (0.35000000000000003, 0.1196) (0.36250000000000004, 0.1185) (0.375, 0.1174) (0.3875, 0.1126) (0.4, 0.1068) (0.41250000000000003, 0.1079) (0.42500000000000004, 0.1076) (0.4375, 0.1077) (0.45, 0.1054) (0.4625, 0.1085) (0.47500000000000003, 0.1052) (0.48750000000000004, 0.1046) (0.5, 0.1048)};
\addlegendentry{456/4}
\end{axis}

==> id40.tex <==
\begin{axis}[anchor=north, no markers, enlargelimits=false, legend columns=2, legend style={draw=none,/tikz/column 2/.style={column sep=5pt,},}, every axis plot/.append style={ultra thick}, legend style = {font=\LARGE,fill=none},ticklabel style={font=\LARGE},title style={font=\LARGE},cycle list name=color list, ytick={0,0.2,0.4,0.6,0.8,1}, yticklabels={,0.2,0.4,0.6,0.8,1}, title= 1D Interval
]
\addplot+[lightgray,forget plot, thick] coordinates{(0,0.5) (0.4,0.5)};
\addplot[red]coordinates{(0.0, 1.0) (0.0125, 0.999) (0.025, 0.9842) (0.037500000000000006, 0.9463) (0.05, 0.896) (0.0625, 0.8507) (0.07500000000000001, 0.7982) (0.08750000000000001, 0.762) (0.1, 0.728) (0.1125, 0.6938) (0.125, 0.671) (0.1375, 0.6423) (0.15000000000000002, 0.6145) (0.1625, 0.5932) (0.17500000000000002, 0.5742) (0.1875, 0.5506) (0.2, 0.5328) (0.21250000000000002, 0.5154) (0.225, 0.4975) (0.23750000000000002, 0.4719) (0.25, 0.4524) (0.2625, 0.4512) (0.275, 0.4349) (0.28750000000000003, 0.4138) (0.30000000000000004, 0.3919) (0.3125, 0.3786) (0.325, 0.3609) (0.3375, 0.3479) (0.35000000000000003, 0.3416) (0.36250000000000004, 0.3243) (0.375, 0.296) (0.3875, 0.2827) (0.4, 0.2706) (0.41250000000000003, 0.2504) (0.42500000000000004, 0.2316) (0.4375, 0.2128) (0.45, 0.1889) (0.4625, 0.1787) (0.47500000000000003, 0.1497) (0.48750000000000004, 0.1287) (0.5, 0.1023)};
\addlegendentry{578/1}
\addplot[blue]coordinates{(0.0, 0.0) (0.0125, 0.0018) (0.025, 0.0212) (0.037500000000000006, 0.0576) (0.05, 0.1037) (0.0625, 0.1408) (0.07500000000000001, 0.1835) (0.08750000000000001, 0.203) (0.1, 0.2212) (0.1125, 0.2328) (0.125, 0.2416) (0.1375, 0.2568) (0.15000000000000002, 0.2592) (0.1625, 0.2641) (0.17500000000000002, 0.2621) (0.1875, 0.2674) (0.2, 0.2712) (0.21250000000000002, 0.2659) (0.225, 0.2636) (0.23750000000000002, 0.2658) (0.25, 0.268) (0.2625, 0.2619) (0.275, 0.2575) (0.28750000000000003, 0.2583) (0.30000000000000004, 0.2574) (0.3125, 0.2499) (0.325, 0.242) (0.3375, 0.2434) (0.35000000000000003, 0.2283) (0.36250000000000004, 0.2286) (0.375, 0.2273) (0.3875, 0.2244) (0.4, 0.2094) (0.41250000000000003, 0.2117) (0.42500000000000004, 0.1956) (0.4375, 0.1795) (0.45, 0.1711) (0.4625, 0.1537) (0.47500000000000003, 0.1433) (0.48750000000000004, 0.1271) (0.5, 0.1007)};
\addlegendentry{558/2}
\addplot[black]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0012) (0.037500000000000006, 0.0049) (0.05, 0.0143) (0.0625, 0.0255) (0.07500000000000001, 0.0365) (0.08750000000000001, 0.049) (0.1, 0.0615) (0.1125, 0.0754) (0.125, 0.0843) (0.1375, 0.0897) (0.15000000000000002, 0.1057) (0.1625, 0.116) (0.17500000000000002, 0.1281) (0.1875, 0.1324) (0.2, 0.1395) (0.21250000000000002, 0.1512) (0.225, 0.1593) (0.23750000000000002, 0.1701) (0.25, 0.1779) (0.2625, 0.1702) (0.275, 0.1806) (0.28750000000000003, 0.1843) (0.30000000000000004, 0.188) (0.3125, 0.1935) (0.325, 0.1973) (0.3375, 0.1998) (0.35000000000000003, 0.1958) (0.36250000000000004, 0.1942) (0.375, 0.193) (0.3875, 0.1872) (0.4, 0.1958) (0.41250000000000003, 0.187) (0.42500000000000004, 0.1737) (0.4375, 0.1732) (0.45, 0.1624) (0.4625, 0.1545) (0.47500000000000003, 0.1412) (0.48750000000000004, 0.1195) (0.5, 0.1012)};
\addlegendentry{551/3}
\addplot[black!30!green]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0) (0.0625, 0.0008) (0.07500000000000001, 0.0034) (0.08750000000000001, 0.0065) (0.1, 0.0096) (0.1125, 0.016) (0.125, 0.0223) (0.1375, 0.0314) (0.15000000000000002, 0.0368) (0.1625, 0.0454) (0.17500000000000002, 0.0522) (0.1875, 0.0625) (0.2, 0.064) (0.21250000000000002, 0.073) (0.225, 0.0817) (0.23750000000000002, 0.0902) (0.25, 0.0941) (0.2625, 0.1018) (0.275, 0.1017) (0.28750000000000003, 0.1121) (0.30000000000000004, 0.1166) (0.3125, 0.124) (0.325, 0.1319) (0.3375, 0.1277) (0.35000000000000003, 0.1384) (0.36250000000000004, 0.1428) (0.375, 0.1457) (0.3875, 0.1462) (0.4, 0.1475) (0.41250000000000003, 0.1463) (0.42500000000000004, 0.1536) (0.4375, 0.1471) (0.45, 0.15) (0.4625, 0.1382) (0.47500000000000003, 0.1347) (0.48750000000000004, 0.1176) (0.5, 0.1054)};
\addlegendentry{531/4}
\end{axis}

==> id42.tex <==
\begin{axis}[anchor=north, no markers, enlargelimits=false, legend columns=2, 
legend style={draw=none,/tikz/column 2/.style={column sep=5pt,},}, every axis 
plot/.append style={ultra thick}, legend style = 
{font=\LARGE,fill=none},ticklabel style={font=\LARGE},title 
style={font=\LARGE},cycle list name=color list, ytick={0,0.2,0.4,0.6,0.8,1}, 
yticklabels={,0.2,0.4,0.6,0.8,1}, title= 1D Interval,label style={font=\huge}, 
	ylabel shift = 3pt, ylabel=$P_c(r)$,xlabel=$r$,xlabel shift = 
	4pt, label 
	style={font=\huge}
]
\addplot+[lightgray,forget plot, thick] coordinates{(0,0.5) (0.5,0.5)};
\addplot[red]coordinates{(0.0, 1.0) (0.0125, 0.9027) (0.025, 0.7697) (0.037500000000000006, 0.6743) (0.05, 0.6015) (0.0625, 0.5505) (0.07500000000000001, 0.5211) (0.08750000000000001, 0.4782) (0.1, 0.4493) (0.1125, 0.4216) (0.125, 0.3896) (0.1375, 0.3608) (0.15000000000000002, 0.3432) (0.1625, 0.3067) (0.17500000000000002, 0.2796) (0.1875, 0.2637) (0.2, 0.2392) (0.21250000000000002, 0.2113) (0.225, 0.1919) (0.23750000000000002, 0.1712) (0.25, 0.152) (0.2625, 0.1422) (0.275, 0.1176) (0.28750000000000003, 0.1052) (0.30000000000000004, 0.103) (0.3125, 0.0933) (0.325, 0.089) (0.3375, 0.0803) (0.35000000000000003, 0.0761) (0.36250000000000004, 0.0701) (0.375, 0.0748) (0.3875, 0.0747) (0.4, 0.0732) (0.41250000000000003, 0.0776) (0.42500000000000004, 0.0801) (0.4375, 0.0814) (0.45, 0.0879) (0.4625, 0.0947) (0.47500000000000003, 0.1001) (0.48750000000000004, 0.1152) (0.5, 0.1245)};
\addlegendentry{23/357/1}
\addplot[blue]coordinates{(0.0, 0.0) (0.0125, 0.1932) (0.025, 0.3245) (0.037500000000000006, 0.416) (0.05, 0.4812) (0.0625, 0.5302) (0.07500000000000001, 0.5531) (0.08750000000000001, 0.5887) (0.1, 0.6073) (0.1125, 0.6111) (0.125, 0.6254) (0.1375, 0.6282) (0.15000000000000002, 0.6177) (0.1625, 0.6142) (0.17500000000000002, 0.5982) (0.1875, 0.571) (0.2, 0.5508) (0.21250000000000002, 0.5121) (0.225, 0.4917) (0.23750000000000002, 0.4644) (0.25, 0.4318) (0.2625, 0.3971) (0.275, 0.3675) (0.28750000000000003, 0.3318) (0.30000000000000004, 0.308) (0.3125, 0.2833) (0.325, 0.2631) (0.3375, 0.2415) (0.35000000000000003, 0.2238) (0.36250000000000004, 0.2121) (0.375, 0.1957) (0.3875, 0.1827) (0.4, 0.1726) (0.41250000000000003, 0.1612) (0.42500000000000004, 0.1582) (0.4375, 0.1442) (0.45, 0.148) (0.4625, 0.1437) (0.47500000000000003, 0.1323) (0.48750000000000004, 0.1325) (0.5, 0.1197)};
\addlegendentry{19/492/2}
\addplot[black]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0003) (0.0625, 0.0005) (0.07500000000000001, 0.0022) (0.08750000000000001, 0.0055) (0.1, 0.0156) (0.1125, 0.0249) (0.125, 0.0424) (0.1375, 0.0609) (0.15000000000000002, 0.0775) (0.1625, 0.1046) (0.17500000000000002, 0.12) (0.1875, 0.1416) (0.2, 0.1656) (0.21250000000000002, 0.1867) (0.225, 0.2042) (0.23750000000000002, 0.2112) (0.25, 0.2192) (0.2625, 0.2253) (0.275, 0.2339) (0.28750000000000003, 0.2384) (0.30000000000000004, 0.2366) (0.3125, 0.231) (0.325, 0.2251) (0.3375, 0.2233) (0.35000000000000003, 0.2206) (0.36250000000000004, 0.211) (0.375, 0.2063) (0.3875, 0.1972) (0.4, 0.1913) (0.41250000000000003, 0.1848) (0.42500000000000004, 0.1706) (0.4375, 0.174) (0.45, 0.1635) (0.4625, 0.1594) (0.47500000000000003, 0.1424) (0.48750000000000004, 0.1357) (0.5, 0.1245)};
\addlegendentry{7/539/6}
\addplot[black!30!green]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0) (0.0625, 0.0) (0.07500000000000001, 0.0) (0.08750000000000001, 0.0001) (0.1, 0.0) (0.1125, 0.0002) (0.125, 0.0006) (0.1375, 0.0018) (0.15000000000000002, 0.005) (0.1625, 0.0098) (0.17500000000000002, 0.0147) (0.1875, 0.0261) (0.2, 0.0347) (0.21250000000000002, 0.0507) (0.225, 0.0613) (0.23750000000000002, 0.0723) (0.25, 0.0891) (0.2625, 0.1032) (0.275, 0.1177) (0.28750000000000003, 0.132) (0.30000000000000004, 0.1328) (0.3125, 0.1437) (0.325, 0.1548) (0.3375, 0.1588) (0.35000000000000003, 0.1693) (0.36250000000000004, 0.168) (0.375, 0.1741) (0.3875, 0.1756) (0.4, 0.1751) (0.41250000000000003, 0.1793) (0.42500000000000004, 0.1719) (0.4375, 0.166) (0.45, 0.164) (0.4625, 0.1468) (0.47500000000000003, 0.1478) (0.48750000000000004, 0.1309) (0.5, 0.1259)};
\addlegendentry{2/546/9}
\end{axis}

==> id459.tex <==
\begin{axis}[anchor=north, no markers, enlargelimits=false, legend columns=2, 
legend style={draw=none,/tikz/column 2/.style={column sep=5pt,},}, every axis 
plot/.append style={ultra thick}, legend style = 
{font=\LARGE,fill=none},ticklabel style={font=\LARGE},title 
style={font=\LARGE},cycle list name=color list, ytick={0,0.2,0.4,0.6,0.8,1}, 
yticklabels={,0.2,0.4,0.6,0.8,1}, title= Urn model 0.2, xlabel=$r$,xlabel shift 
= 4pt, label style={font=\huge}
]
\addplot+[lightgray,forget plot, thick] coordinates{(0,0.5) (0.4,0.5)};
\addplot[red]coordinates{(0.0, 1.0) (0.0125, 0.935) (0.025, 0.9166) (0.037500000000000006, 0.9038) (0.05, 0.8844) (0.0625, 0.8723) (0.07500000000000001, 0.8582) (0.08750000000000001, 0.8397) (0.1, 0.8288) (0.1125, 0.807) (0.125, 0.7825) (0.1375, 0.7706) (0.15000000000000002, 0.7487) (0.1625, 0.7222) (0.17500000000000002, 0.7008) (0.1875, 0.6741) (0.2, 0.6647) (0.21250000000000002, 0.6388) (0.225, 0.6244) (0.23750000000000002, 0.6117) (0.25, 0.5861) (0.2625, 0.57) (0.275, 0.5605) (0.28750000000000003, 0.5296) (0.30000000000000004, 0.5278) (0.3125, 0.5051) (0.325, 0.491) (0.3375, 0.478) (0.35000000000000003, 0.4683) (0.36250000000000004, 0.4468) (0.375, 0.4265) (0.3875, 0.419) (0.4, 0.3946) (0.41250000000000003, 0.3896) (0.42500000000000004, 0.3557) (0.4375, 0.3445) (0.45, 0.293) (0.4625, 0.2629) (0.47500000000000003, 0.2038) (0.48750000000000004, 0.1597) (0.5, 0.0919)};
\addlegendentry{707/1}
\addplot[blue]coordinates{(0.0, 0.0) (0.0125, 0.0958) (0.025, 0.1092) (0.037500000000000006, 0.1183) (0.05, 0.1323) (0.0625, 0.1462) (0.07500000000000001, 0.1584) (0.08750000000000001, 0.1747) (0.1, 0.1853) (0.1125, 0.2091) (0.125, 0.2323) (0.1375, 0.2399) (0.15000000000000002, 0.2627) (0.1625, 0.2883) (0.17500000000000002, 0.3062) (0.1875, 0.3279) (0.2, 0.3343) (0.21250000000000002, 0.3547) (0.225, 0.3619) (0.23750000000000002, 0.3672) (0.25, 0.3854) (0.2625, 0.3933) (0.275, 0.391) (0.28750000000000003, 0.4116) (0.30000000000000004, 0.4007) (0.3125, 0.4146) (0.325, 0.4138) (0.3375, 0.4106) (0.35000000000000003, 0.4064) (0.36250000000000004, 0.4024) (0.375, 0.4044) (0.3875, 0.3875) (0.4, 0.3756) (0.41250000000000003, 0.3579) (0.42500000000000004, 0.3478) (0.4375, 0.3126) (0.45, 0.2882) (0.4625, 0.2525) (0.47500000000000003, 0.2118) (0.48750000000000004, 0.1462) (0.5, 0.0993)};
\addlegendentry{703/2}
\addplot[black]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0) (0.0625, 0.0) (0.07500000000000001, 0.0) (0.08750000000000001, 0.0) (0.1, 0.0) (0.1125, 0.0002) (0.125, 0.0007) (0.1375, 0.0015) (0.15000000000000002, 0.0022) (0.1625, 0.0045) (0.17500000000000002, 0.007) (0.1875, 0.0117) (0.2, 0.0151) (0.21250000000000002, 0.0201) (0.225, 0.025) (0.23750000000000002, 0.0337) (0.25, 0.0436) (0.2625, 0.0514) (0.275, 0.0632) (0.28750000000000003, 0.0714) (0.30000000000000004, 0.0867) (0.3125, 0.0928) (0.325, 0.1063) (0.3375, 0.1218) (0.35000000000000003, 0.1327) (0.36250000000000004, 0.1503) (0.375, 0.165) (0.3875, 0.1732) (0.4, 0.1941) (0.41250000000000003, 0.1935) (0.42500000000000004, 0.2064) (0.4375, 0.2047) (0.45, 0.2096) (0.4625, 0.1929) (0.47500000000000003, 0.175) (0.48750000000000004, 0.1409) (0.5, 0.1045)};
\addlegendentry{642/3}
\addplot[black!30!green]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0) (0.0625, 0.0) (0.07500000000000001, 0.0) (0.08750000000000001, 0.0) (0.1, 0.0) (0.1125, 0.0) (0.125, 0.0) (0.1375, 0.0) (0.15000000000000002, 0.0) (0.1625, 0.0) (0.17500000000000002, 0.0) (0.1875, 0.0) (0.2, 0.0) (0.21250000000000002, 0.0) (0.225, 0.0) (0.23750000000000002, 0.0) (0.25, 0.0) (0.2625, 0.0) (0.275, 0.0) (0.28750000000000003, 0.0002) (0.30000000000000004, 0.0003) (0.3125, 0.0008) (0.325, 0.0015) (0.3375, 0.0037) (0.35000000000000003, 0.0036) (0.36250000000000004, 0.0088) (0.375, 0.0126) (0.3875, 0.0212) (0.4, 0.0262) (0.41250000000000003, 0.0382) (0.42500000000000004, 0.0533) (0.4375, 0.0616) (0.45, 0.0864) (0.4625, 0.1009) (0.47500000000000003, 0.1144) (0.48750000000000004, 0.1167) (0.5, 0.1084)};
\addlegendentry{518/4}
\end{axis}

==> id491.tex <==
\begin{axis}[anchor=north, no markers, enlargelimits=false, legend columns=2, 
legend style={draw=none,/tikz/column 2/.style={column sep=5pt,},}, every axis 
plot/.append style={ultra thick}, legend style = 
{font=\LARGE,fill=none},ticklabel style={font=\LARGE},title 
style={font=\LARGE},cycle list name=color list, ytick={0,0.2,0.4,0.6,0.8,1}, 
yticklabels={,0.2,0.4,0.6,0.8,1}, title= Urn model 0.1, xlabel=$r$,xlabel shift 
= 4pt, label style={font=\huge}
]
\addplot+[lightgray,forget plot, thick] coordinates{(0,0.5) (0.5,0.5)};
\addplot[red]coordinates{(0.0, 1.0) (0.0125, 1.0) (0.025, 1.0) (0.037500000000000006, 1.0) (0.05, 1.0) (0.0625, 0.9998) (0.07500000000000001, 0.9985) (0.08750000000000001, 0.9956) (0.1, 0.9868) (0.1125, 0.9756) (0.125, 0.9519) (0.1375, 0.9302) (0.15000000000000002, 0.899) (0.1625, 0.8581) (0.17500000000000002, 0.825) (0.1875, 0.7768) (0.2, 0.75) (0.21250000000000002, 0.706) (0.225, 0.6751) (0.23750000000000002, 0.6413) (0.25, 0.6158) (0.2625, 0.5777) (0.275, 0.5429) (0.28750000000000003, 0.5134) (0.30000000000000004, 0.4778) (0.3125, 0.4564) (0.325, 0.4302) (0.3375, 0.4033) (0.35000000000000003, 0.372) (0.36250000000000004, 0.3551) (0.375, 0.3217) (0.3875, 0.2968) (0.4, 0.2748) (0.41250000000000003, 0.2527) (0.42500000000000004, 0.2338) (0.4375, 0.2112) (0.45, 0.1945) (0.4625, 0.1713) (0.47500000000000003, 0.1497) (0.48750000000000004, 0.1326) (0.5, 0.1235)};
\addlegendentry{41/573/1}
\addplot[blue]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0) (0.0625, 0.0) (0.07500000000000001, 0.0) (0.08750000000000001, 0.0) (0.1, 0.0) (0.1125, 0.0001) (0.125, 0.0003) (0.1375, 0.0006) (0.15000000000000002, 0.0007) (0.1625, 0.0023) (0.17500000000000002, 0.0033) (0.1875, 0.0069) (0.2, 0.0102) (0.21250000000000002, 0.0148) (0.225, 0.0204) (0.23750000000000002, 0.0278) (0.25, 0.0357) (0.2625, 0.0475) (0.275, 0.0555) (0.28750000000000003, 0.0666) (0.30000000000000004, 0.0749) (0.3125, 0.0884) (0.325, 0.1007) (0.3375, 0.1092) (0.35000000000000003, 0.1165) (0.36250000000000004, 0.1197) (0.375, 0.1358) (0.3875, 0.1369) (0.4, 0.1477) (0.41250000000000003, 0.1519) (0.42500000000000004, 0.1513) (0.4375, 0.1528) (0.45, 0.1515) (0.4625, 0.1475) (0.47500000000000003, 0.1307) (0.48750000000000004, 0.1329) (0.5, 0.1256)};
\addlegendentry{7/512/5}
\addplot[black]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0) (0.0625, 0.0) (0.07500000000000001, 0.0) (0.08750000000000001, 0.0) (0.1, 0.0) (0.1125, 0.0) (0.125, 0.0) (0.1375, 0.0) (0.15000000000000002, 0.0) (0.1625, 0.0) (0.17500000000000002, 0.0) (0.1875, 0.0) (0.2, 0.0004) (0.21250000000000002, 0.0007) (0.225, 0.0007) (0.23750000000000002, 0.0017) (0.25, 0.0048) (0.2625, 0.0068) (0.275, 0.0103) (0.28750000000000003, 0.0126) (0.30000000000000004, 0.0199) (0.3125, 0.0269) (0.325, 0.0303) (0.3375, 0.0457) (0.35000000000000003, 0.0552) (0.36250000000000004, 0.0645) (0.375, 0.0752) (0.3875, 0.0815) (0.4, 0.0932) (0.41250000000000003, 0.1034) (0.42500000000000004, 0.1099) (0.4375, 0.1084) (0.45, 0.1192) (0.4625, 0.1226) (0.47500000000000003, 0.1205) (0.48750000000000004, 0.1316) (0.5, 0.1251)};
\addlegendentry{1/468/9}
\addplot[black!30!green]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0) (0.0625, 0.0003) (0.07500000000000001, 0.0028) (0.08750000000000001, 0.0072) (0.1, 0.0199) (0.1125, 0.0361) (0.125, 0.065) (0.1375, 0.0928) (0.15000000000000002, 0.1348) (0.1625, 0.1841) (0.17500000000000002, 0.2185) (0.1875, 0.2696) (0.2, 0.2958) (0.21250000000000002, 0.3434) (0.225, 0.3736) (0.23750000000000002, 0.3947) (0.25, 0.4191) (0.2625, 0.4337) (0.275, 0.4586) (0.28750000000000003, 0.4627) (0.30000000000000004, 0.4795) (0.3125, 0.4771) (0.325, 0.4675) (0.3375, 0.4528) (0.35000000000000003, 0.4417) (0.36250000000000004, 0.4243) (0.375, 0.3954) (0.3875, 0.3812) (0.4, 0.3461) (0.41250000000000003, 0.3305) (0.42500000000000004, 0.2849) (0.4375, 0.2592) (0.45, 0.231) (0.4625, 0.2001) (0.47500000000000003, 0.1727) (0.48750000000000004, 0.147) (0.5, 0.1258)};
\addlegendentry{0/638/10}
\end{axis}

==> id504.tex <==
\begin{axis}[anchor=north, no markers, enlargelimits=false, legend columns=2, 
legend style={draw=none,/tikz/column 2/.style={column sep=5pt,},}, every axis 
plot/.append style={ultra thick}, legend style = 
{font=\LARGE,fill=none},ticklabel style={font=\LARGE},title 
style={font=\LARGE},cycle list name=color list, ytick={0,0.2,0.4,0.6,0.8,1}, 
yticklabels={,0.2,0.4,0.6,0.8,1}, title= Urn model 0.1,label 
style={font=\huge}, 
	ylabel shift = 3pt, ylabel=$P_c(r)$, xlabel=$r$,xlabel shift = 4pt
]
\addplot+[lightgray,forget plot, thick] coordinates{(0,0.5) (0.4,0.5)};
\addplot[red]coordinates{(0.0, 1.0) (0.0125, 0.5207) (0.025, 0.4307) (0.037500000000000006, 0.39) (0.05, 0.3673) (0.0625, 0.377) (0.07500000000000001, 0.3653) (0.08750000000000001, 0.3775) (0.1, 0.3773) (0.1125, 0.3856) (0.125, 0.3906) (0.1375, 0.3969) (0.15000000000000002, 0.3982) (0.1625, 0.4175) (0.17500000000000002, 0.4186) (0.1875, 0.422) (0.2, 0.4179) (0.21250000000000002, 0.4269) (0.225, 0.4286) (0.23750000000000002, 0.4291) (0.25, 0.4281) (0.2625, 0.4303) (0.275, 0.4188) (0.28750000000000003, 0.4153) (0.30000000000000004, 0.4104) (0.3125, 0.4138) (0.325, 0.3993) (0.3375, 0.3884) (0.35000000000000003, 0.3827) (0.36250000000000004, 0.364) (0.375, 0.353) (0.3875, 0.3375) (0.4, 0.3133) (0.41250000000000003, 0.2865) (0.42500000000000004, 0.2666) (0.4375, 0.2403) (0.45, 0.2152) (0.4625, 0.182) (0.47500000000000003, 0.1582) (0.48750000000000004, 0.1225) (0.5, 0.1042)};
\addlegendentry{577/1}
\addplot[blue]coordinates{(0.0, 0.0) (0.0125, 0.5561) (0.025, 0.62) (0.037500000000000006, 0.6482) (0.05, 0.6658) (0.0625, 0.6525) (0.07500000000000001, 0.6602) (0.08750000000000001, 0.6417) (0.1, 0.6427) (0.1125, 0.6268) (0.125, 0.6163) (0.1375, 0.5992) (0.15000000000000002, 0.59) (0.1625, 0.5672) (0.17500000000000002, 0.5565) (0.1875, 0.5432) (0.2, 0.5355) (0.21250000000000002, 0.5151) (0.225, 0.4957) (0.23750000000000002, 0.4944) (0.25, 0.4782) (0.2625, 0.4578) (0.275, 0.4654) (0.28750000000000003, 0.4451) (0.30000000000000004, 0.4316) (0.3125, 0.4217) (0.325, 0.4101) (0.3375, 0.4059) (0.35000000000000003, 0.3862) (0.36250000000000004, 0.369) (0.375, 0.3537) (0.3875, 0.3362) (0.4, 0.3137) (0.41250000000000003, 0.2888) (0.42500000000000004, 0.2712) (0.4375, 0.2359) (0.45, 0.2131) (0.4625, 0.1837) (0.47500000000000003, 0.1529) (0.48750000000000004, 0.126) (0.5, 0.1008)};
\addlegendentry{575/2}
\addplot[black]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0) (0.0625, 0.0002) (0.07500000000000001, 0.0009) (0.08750000000000001, 0.0024) (0.1, 0.0051) (0.1125, 0.0084) (0.125, 0.014) (0.1375, 0.0223) (0.15000000000000002, 0.0271) (0.1625, 0.0329) (0.17500000000000002, 0.0425) (0.1875, 0.0539) (0.2, 0.0635) (0.21250000000000002, 0.0727) (0.225, 0.0876) (0.23750000000000002, 0.0891) (0.25, 0.1032) (0.2625, 0.1186) (0.275, 0.1209) (0.28750000000000003, 0.1399) (0.30000000000000004, 0.1474) (0.3125, 0.1521) (0.325, 0.164) (0.3375, 0.1677) (0.35000000000000003, 0.1765) (0.36250000000000004, 0.1838) (0.375, 0.1952) (0.3875, 0.1913) (0.4, 0.1926) (0.41250000000000003, 0.1924) (0.42500000000000004, 0.1767) (0.4375, 0.1725) (0.45, 0.1664) (0.4625, 0.1479) (0.47500000000000003, 0.1354) (0.48750000000000004, 0.1203) (0.5, 0.0977)};
\addlegendentry{535/3}
\addplot[black!30!green]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0) (0.0625, 0.0) (0.07500000000000001, 0.0) (0.08750000000000001, 0.0) (0.1, 0.0) (0.1125, 0.0) (0.125, 0.0) (0.1375, 0.0) (0.15000000000000002, 0.0) (0.1625, 0.0) (0.17500000000000002, 0.0004) (0.1875, 0.0004) (0.2, 0.0013) (0.21250000000000002, 0.0013) (0.225, 0.0031) (0.23750000000000002, 0.0047) (0.25, 0.0055) (0.2625, 0.01) (0.275, 0.0113) (0.28750000000000003, 0.0159) (0.30000000000000004, 0.0247) (0.3125, 0.0255) (0.325, 0.0346) (0.3375, 0.0398) (0.35000000000000003, 0.0522) (0.36250000000000004, 0.0673) (0.375, 0.0695) (0.3875, 0.081) (0.4, 0.0945) (0.41250000000000003, 0.0952) (0.42500000000000004, 0.1053) (0.4375, 0.1078) (0.45, 0.1086) (0.4625, 0.1131) (0.47500000000000003, 0.113) (0.48750000000000004, 0.1087) (0.5, 0.105)};
\addlegendentry{482/4}
\end{axis}

==> id537.tex <==
\begin{axis}[anchor=north, no markers, enlargelimits=false, legend columns=2, 
legend style={draw=none,/tikz/column 2/.style={column sep=5pt,},}, every axis 
plot/.append style={ultra thick}, legend style = 
{font=\LARGE,fill=none},ticklabel style={font=\LARGE},title 
style={font=\LARGE},cycle list name=color list, ytick={0,0.2,0.4,0.6,0.8,1}, 
yticklabels={,0.2,0.4,0.6,0.8,1}, title= Urn model 0.05
]
\addplot+[lightgray,forget plot, thick] coordinates{(0,0.5) (0.5,0.5)};
\addplot[red]coordinates{(0.0, 1.0) (0.0125, 0.979) (0.025, 0.9626) (0.037500000000000006, 0.9558) (0.05, 0.9562) (0.0625, 0.9515) (0.07500000000000001, 0.9497) (0.08750000000000001, 0.944) (0.1, 0.9438) (0.1125, 0.9367) (0.125, 0.9296) (0.1375, 0.9324) (0.15000000000000002, 0.9227) (0.1625, 0.9074) (0.17500000000000002, 0.9037) (0.1875, 0.8863) (0.2, 0.868) (0.21250000000000002, 0.8462) (0.225, 0.8323) (0.23750000000000002, 0.8166) (0.25, 0.7802) (0.2625, 0.7551) (0.275, 0.7389) (0.28750000000000003, 0.7122) (0.30000000000000004, 0.6777) (0.3125, 0.6489) (0.325, 0.6114) (0.3375, 0.5871) (0.35000000000000003, 0.5558) (0.36250000000000004, 0.5056) (0.375, 0.4701) (0.3875, 0.4473) (0.4, 0.4011) (0.41250000000000003, 0.3605) (0.42500000000000004, 0.3231) (0.4375, 0.288) (0.45, 0.2441) (0.4625, 0.2131) (0.47500000000000003, 0.1782) (0.48750000000000004, 0.1542) (0.5, 0.1267)};
\addlegendentry{31/662/1}
\addplot[blue]coordinates{(0.0, 0.0) (0.0125, 0.0589) (0.025, 0.0703) (0.037500000000000006, 0.0736) (0.05, 0.0731) (0.0625, 0.0772) (0.07500000000000001, 0.0765) (0.08750000000000001, 0.0807) (0.1, 0.0815) (0.1125, 0.0915) (0.125, 0.0942) (0.1375, 0.0943) (0.15000000000000002, 0.1026) (0.1625, 0.1124) (0.17500000000000002, 0.1158) (0.1875, 0.13) (0.2, 0.1323) (0.21250000000000002, 0.1461) (0.225, 0.1446) (0.23750000000000002, 0.1502) (0.25, 0.1683) (0.2625, 0.1739) (0.275, 0.1737) (0.28750000000000003, 0.1905) (0.30000000000000004, 0.1986) (0.3125, 0.201) (0.325, 0.2076) (0.3375, 0.2054) (0.35000000000000003, 0.2078) (0.36250000000000004, 0.2096) (0.375, 0.2148) (0.3875, 0.2116) (0.4, 0.2103) (0.41250000000000003, 0.207) (0.42500000000000004, 0.2001) (0.4375, 0.1869) (0.45, 0.1732) (0.4625, 0.1616) (0.47500000000000003, 0.1518) (0.48750000000000004, 0.1359) (0.5, 0.1255)};
\addlegendentry{28/564/2}
\addplot[black]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0) (0.0625, 0.0) (0.07500000000000001, 0.0) (0.08750000000000001, 0.0) (0.1, 0.0) (0.1125, 0.0) (0.125, 0.0) (0.1375, 0.0) (0.15000000000000002, 0.0001) (0.1625, 0.0004) (0.17500000000000002, 0.0) (0.1875, 0.0006) (0.2, 0.0018) (0.21250000000000002, 0.0026) (0.225, 0.0028) (0.23750000000000002, 0.0045) (0.25, 0.0073) (0.2625, 0.0107) (0.275, 0.0131) (0.28750000000000003, 0.0175) (0.30000000000000004, 0.0253) (0.3125, 0.029) (0.325, 0.0365) (0.3375, 0.0441) (0.35000000000000003, 0.0534) (0.36250000000000004, 0.0608) (0.375, 0.0794) (0.3875, 0.0783) (0.4, 0.0924) (0.41250000000000003, 0.1012) (0.42500000000000004, 0.1086) (0.4375, 0.1162) (0.45, 0.1222) (0.4625, 0.1248) (0.47500000000000003, 0.124) (0.48750000000000004, 0.1246) (0.5, 0.1261)};
\addlegendentry{13/465/3}
\addplot[black!30!green]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0) (0.0625, 0.0) (0.07500000000000001, 0.0) (0.08750000000000001, 0.0) (0.1, 0.0001) (0.1125, 0.0006) (0.125, 0.002) (0.1375, 0.0043) (0.15000000000000002, 0.0098) (0.1625, 0.0131) (0.17500000000000002, 0.0213) (0.1875, 0.029) (0.2, 0.0435) (0.21250000000000002, 0.0613) (0.225, 0.0768) (0.23750000000000002, 0.0859) (0.25, 0.1041) (0.2625, 0.1311) (0.275, 0.1457) (0.28750000000000003, 0.1569) (0.30000000000000004, 0.1732) (0.3125, 0.1969) (0.325, 0.208) (0.3375, 0.2181) (0.35000000000000003, 0.2291) (0.36250000000000004, 0.2429) (0.375, 0.2374) (0.3875, 0.2415) (0.4, 0.2348) (0.41250000000000003, 0.2324) (0.42500000000000004, 0.2229) (0.4375, 0.2078) (0.45, 0.1975) (0.4625, 0.1795) (0.47500000000000003, 0.1611) (0.48750000000000004, 0.1382) (0.5, 0.1264)};
\addlegendentry{7/603/5}
\end{axis}

==> id661.tex <==
\begin{axis}[anchor=north, no markers, enlargelimits=false, legend columns=2, 
legend style={draw=none,/tikz/column 2/.style={column sep=5pt,},}, every axis 
plot/.append style={ultra thick}, legend style = 
{font=\LARGE,fill=none},ticklabel style={font=\LARGE},title 
style={font=\LARGE},cycle list name=color list, ytick={0,0.2,0.4,0.6,0.8,1}, 
yticklabels={,0.2,0.4,0.6,0.8,1}, title= Mallows 0.75,label style={font=\huge}, 
	ylabel shift = 3pt, ylabel=$P_c(r)$
]
\addplot+[lightgray,forget plot, thick] coordinates{(0,0.5) (0.4,0.5)};
\addplot[red]coordinates{(0.0, 1.0) (0.0125, 1.0) (0.025, 1.0) (0.037500000000000006, 1.0) (0.05, 1.0) (0.0625, 0.9998) (0.07500000000000001, 0.9985) (0.08750000000000001, 0.996) (0.1, 0.9908) (0.1125, 0.9833) (0.125, 0.9706) (0.1375, 0.9616) (0.15000000000000002, 0.9485) (0.1625, 0.9357) (0.17500000000000002, 0.9169) (0.1875, 0.8979) (0.2, 0.8847) (0.21250000000000002, 0.8685) (0.225, 0.8479) (0.23750000000000002, 0.8297) (0.25, 0.807) (0.2625, 0.7829) (0.275, 0.7649) (0.28750000000000003, 0.7425) (0.30000000000000004, 0.7154) (0.3125, 0.6926) (0.325, 0.6609) (0.3375, 0.6313) (0.35000000000000003, 0.6083) (0.36250000000000004, 0.5593) (0.375, 0.5355) (0.3875, 0.497) (0.4, 0.4632) (0.41250000000000003, 0.4249) (0.42500000000000004, 0.3749) (0.4375, 0.3427) (0.45, 0.2937) (0.4625, 0.2389) (0.47500000000000003, 0.1896) (0.48750000000000004, 0.1468) (0.5, 0.0925)};
\addlegendentry{652/1}
\addplot[blue]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0) (0.0625, 0.0004) (0.07500000000000001, 0.0018) (0.08750000000000001, 0.0048) (0.1, 0.0107) (0.1125, 0.0191) (0.125, 0.032) (0.1375, 0.0418) (0.15000000000000002, 0.0557) (0.1625, 0.0692) (0.17500000000000002, 0.0881) (0.1875, 0.1058) (0.2, 0.1157) (0.21250000000000002, 0.1308) (0.225, 0.1481) (0.23750000000000002, 0.1628) (0.25, 0.1781) (0.2625, 0.1951) (0.275, 0.2053) (0.28750000000000003, 0.2195) (0.30000000000000004, 0.2291) (0.3125, 0.2391) (0.325, 0.2483) (0.3375, 0.2535) (0.35000000000000003, 0.2597) (0.36250000000000004, 0.2655) (0.375, 0.264) (0.3875, 0.2672) (0.4, 0.2555) (0.41250000000000003, 0.2531) (0.42500000000000004, 0.2489) (0.4375, 0.2297) (0.45, 0.2015) (0.4625, 0.1906) (0.47500000000000003, 0.1566) (0.48750000000000004, 0.1276) (0.5, 0.1064)};
\addlegendentry{601/2}
\addplot[black]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0) (0.0625, 0.0) (0.07500000000000001, 0.0) (0.08750000000000001, 0.0) (0.1, 0.0) (0.1125, 0.0) (0.125, 0.0) (0.1375, 0.0) (0.15000000000000002, 0.0001) (0.1625, 0.0006) (0.17500000000000002, 0.0009) (0.1875, 0.0035) (0.2, 0.0062) (0.21250000000000002, 0.0079) (0.225, 0.0103) (0.23750000000000002, 0.0161) (0.25, 0.0219) (0.2625, 0.0277) (0.275, 0.0357) (0.28750000000000003, 0.0412) (0.30000000000000004, 0.0571) (0.3125, 0.0621) (0.325, 0.0778) (0.3375, 0.0908) (0.35000000000000003, 0.0991) (0.36250000000000004, 0.1193) (0.375, 0.1232) (0.3875, 0.1342) (0.4, 0.1459) (0.41250000000000003, 0.1484) (0.42500000000000004, 0.1542) (0.4375, 0.1606) (0.45, 0.1599) (0.4625, 0.1524) (0.47500000000000003, 0.1389) (0.48750000000000004, 0.1191) (0.5, 0.1112)};
\addlegendentry{555/3}
\addplot[black!30!green]coordinates{(0.0, 0.0) (0.0125, 0.0) (0.025, 0.0) (0.037500000000000006, 0.0) (0.05, 0.0) (0.0625, 0.0) (0.07500000000000001, 0.0) (0.08750000000000001, 0.0) (0.1, 0.0) (0.1125, 0.0) (0.125, 0.0) (0.1375, 0.0) (0.15000000000000002, 0.0) (0.1625, 0.0) (0.17500000000000002, 0.0) (0.1875, 0.0) (0.2, 0.0) (0.21250000000000002, 0.0001) (0.225, 0.0001) (0.23750000000000002, 0.0004) (0.25, 0.0007) (0.2625, 0.0011) (0.275, 0.0029) (0.28750000000000003, 0.0049) (0.30000000000000004, 0.0074) (0.3125, 0.011) (0.325, 0.016) (0.3375, 0.0222) (0.35000000000000003, 0.0265) (0.36250000000000004, 0.0377) (0.375, 0.0481) (0.3875, 0.0581) (0.4, 0.0674) (0.41250000000000003, 0.078) (0.42500000000000004, 0.0889) (0.4375, 0.0951) (0.45, 0.1096) (0.4625, 0.1121) (0.47500000000000003, 0.1156) (0.48750000000000004, 0.1161) (0.5, 0.104)};
\addlegendentry{506/4}
\end{axis}
